KANs need curvature: penalties for compositional smoothness

Kolmogorov-Arnold networks (KANs) offer a potent combination of accuracy and interpretability, thanks to their compositions of learnable univariate activation functions. However, the activations of well-fitting KANs tend to exhibit pathologically high-curvature oscillations, making them difficult to interpret, and standard regularization penalties do not prevent this. Here we derive a basis-agnostic curvature penalty and show that penalized models can maintain accuracy while achieving substantially smoother activations. Accounting for how function composition shapes curvature, we prove an upper bound on the full model's curvature relative to the curvature penalty, and use this to motivate richer forms of penalties. Scientific machine learning is increasingly bottlenecked by the trade-off between accuracy and interpretability. Results such as ours that improve interpretability without sacrificing accuracy will further strengthen KANs as a practical tool for both prediction and insight.

==> tab_feynman.tex <==
\begin{table*}[ht]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{l l ccc c ccc}
    \toprule
    & & \multicolumn{3}{c}{Test RMSE (median)} & & \multicolumn{3}{c}{$\sum_e\!\int(\phi_e'')^2$ (median)} \\
    \cmidrule(lr){3-5} \cmidrule(lr){7-9}
    Feynman eq.\ & Formula & No penalty & KAN & Curvature & & No penalty & KAN & Curvature \\
    \midrule
    I.6.20 & $e^{-\theta^2/(2\sigma^2)} / \sqrt{2\pi\sigma^2}$ & \textbf{0.0015} & \textit{0.0022} & 0.0034 & & $52.7$ & $305$ & $\mathbf{17.7}$ \\
    I.6.20b & $e^{-(\theta-\theta_1)^2/(2\sigma^2)} / \sqrt{2\pi\sigma^2}$ & \textbf{0.0058} & \textit{0.0075} & \textit{0.0070} & & $74.8$ & $107$ & $\mathbf{11.8}$ \\
    I.9.18 & $G m_1 m_2 / \big[(\Delta x)^2 + (\Delta y)^2 + (\Delta z)^2\big]$ & \textbf{0.0022} & 0.0069 & \textit{0.0022} & & $118$ & $1.2\!\cdot\!10^{4}$ & $\mathbf{14.7}$ \\
    I.12.11 & $q\,(E_f + B v \sin\theta)$ & \textit{0.0751} & \textit{0.0720} & \textbf{0.0560} & & $112$ & $99.5$ & $\mathbf{36.6}$ \\
    I.16.6 & $uv / (1 + uv/c^2)$ & \textbf{0.0061} & \textit{0.0075} & \textit{0.0070} & & $179$ & $278$ & $\mathbf{29.0}$ \\
    I.18.4 & $(m_1 r_1 + m_2 r_2) / (m_1 + m_2)$ & \textit{0.0013} & 0.0023 & \textbf{0.0009} & & $60.2$ & $480$ & $\mathbf{29.0}$ \\
    I.26.2 & $\arcsin(n \sin\theta_2)$ & \textbf{0.0094} & \textit{0.0098} & \textit{0.0136} & & $84.7$ & $72.3$ & $\mathbf{19.2}$ \\
    I.29.16 & $\sqrt{x_1^2 + x_2^2 - 2 x_1 x_2 \cos(\theta_1-\theta_2)}$ & \textbf{0.1256} & \textit{0.1527} & \textit{0.1294} & & $390$ & $393$ & $\mathbf{63.1}$ \\
    I.30.3 & $I_0\,\sin^2(n\theta/2) / \sin^2(\theta/2)$ & \textit{0.1787} & \textit{0.1789} & \textbf{0.1763} & & $619$ & $559$ & $\mathbf{153}$ \\
    I.50.26 & $x_1\,[\cos(\omega t) + \alpha\cos^2(\omega t)]$ & \textbf{0.0365} & \textit{0.0367} & \textit{0.0450} & & $194$ & $136$ & $\mathbf{67.9}$ \\
    II.11.27 & $n\alpha\,\epsilon E_f / (1 - n\alpha/3)$ & \textit{0.0085} & \textbf{0.0076} & \textit{0.0084} & & $766$ & $1088$ & $\mathbf{627}$ \\
    II.35.18 & $n_0 / [\,e^{\mu B/k_b T} + e^{-\mu B/k_b T}\,]$ & \textbf{0.0016} & 0.0056 & \textit{0.0018} & & $51.5$ & $2.1\!\cdot\!10^{6}$ & $\mathbf{19.6}$ \\
    III.10.19 & $\mu\,\sqrt{B_x^2 + B_y^2 + B_z^2}$ & \textbf{0.0038} & 0.0081 & \textit{0.0054} & & $2340$ & $2744$ & $\mathbf{258}$ \\
    III.17.37 & $\beta\,(1 + \alpha \cos\theta)$ & \textbf{0.0089} & \textit{0.0095} & \textit{0.0161} & & $95.4$ & $76.3$ & $\mathbf{20.4}$ \\
    \bottomrule
  \end{tabular}
  \caption{Feynman benchmark, $G=10$, $n=5$ seeds, architecture $[d_{\text{in}}, d_{\text{in}}, 1]$. Each penalty is shown at the single $\lambda^*$ that minimizes the geometric mean of test RMSE across all 14 equations: $\lambda^*=0.0001$ for the KAN penalty and $\lambda^*=0.0001$ for the curvature penalty. Winner in each RMSE block bolded per row; non-winners within $2\times$ the winner italicized. Curvature winner bolded per row. The curvature penalty matches or beats the KAN penalty on median RMSE in 9/14 equations and has the lowest total edge curvature in 14/14.}
  \label{tab:feynman}
\end{table*}

